Effect of freestream turbulence on the coherent dynamics of a wind turbine wake

The wake of a model wind turbine exposed to incoming freestream turbulence (FST) with a variety of turbulent characteristics is studied through Particle Image Velocimetry experiments. The FST cases were produced using different passive turbulence generating grids. The cases spanned turbulent intensities (T<sub>i</sub>) in the range 1.3% < T<sub>i</sub> < 14% and only considered short integral length scales L<sub>v</sub><0.2D (where D is the turbine diameter). Increasing T<sub>i</sub> and L<sub>v</sub> in this range resulted in an earlier breakdown of the tip vortices which in turn resulted in an earlier onset of wake recovery. For all the FST cases considered, the initiation of wake meandering was found to be related to an intrinsic instability of the turbine, even for the cases with the highest FST levels. The amplitudes of wake meandering were similar for all the cases in the near wake (x<2D), but the amplitudes in the far wake (x>4D) were discernibly higher for all the FST cases compared to the no grid case (lowest T<sub>i</sub>), primarily due to the early break down of the tip vortices. Deeper insights into the origins, and subsequent evolution, of the various coherent motions (characterised by particular frequencies) in the presence of FST are obtained through analysis of the multi-scale triple-decomposed coherent kinetic energy budgets. The wake meandering modes in the presence of FST are shown to better utilize the mean velocity shear, extracting more energy from the mean flow while other sources such as non-linear triadic interactions and diffusion also become important.

==> README <==

  The ulem package provides various types of underlining that can stretch
  between words and be broken across lines in LaTeX or plain TeX.
  In LaTeX ulem replaces italics with underlining in \em-phasized text.
  A declaration of \normalem (or the \usepackage option "normalem") restores 
  the normal \em and \emph behavior.

  Copyright 1989-2019 by Donald Arseneau (Vancouver, Canada; asnd@triumf.ca)

  This software may be freely transmitted, reproduced, or modified for any
  purpose provided that this copyright notice is left intact.  

